Estimation of the covariate conditional tail expectation : a depth-based level set approach

The aim of this paper is to study the asymptotic behavior of a particular multivariate risk measure, the Covariate-Conditional-Tail-Expectation (CCTE), based on a multivariate statistical depth function. Depth functions have become increasingly powerful tools in nonparametric inference for multivariate data, as they measure a degree of centrality of a point with respect to a distribution. A multivariate risks scenario is then represented by a depth-based lower level set of the risk factors, meaning that we consider a non-compact setting. More precisely, given a multivariate depth function D associated to a fixed probability measure, we are interested in the lower level set based on D. First, we present a plug-in approach in order to estimate the depth-based level set. In a second part, we provide a consistent estimator of our CCTE for a general depth function with a rate of convergence, and we consider the particular case of the Mahalanobis depth. A simulation study complements the performances of our estimator.

==> bordasymptotique.tex <==
\begin{tikzpicture}
%\draw [domain=-1:2\pi,samples=200,color=blue,very thick] plot ({2*cos(\x)},{2*sin(\x)});
%tracer le plan (x,y)
\draw[->] (-4,-1) -- (5,-1) node[below right] {$x$};
\draw[->] (-3,-2) -- (-3,4) node[left] {$y$};

\filldraw[color=red!60, fill=green!2, thick,rotate=45](2.5,0) ellipse (2 and 1.5);
\filldraw[very thick] (2,2) node{$(\mathring{\mathcal{L}_n})^c$};
\draw[very thick] (-2,0.8) node{$\mathcal{L}_n$};
\filldraw[very thick,color=red]  (0,3) node{$\partial \mathcal{L}_n$};
\draw[dashed] (-1,0) -- (1,1.4);
\draw (-1,0) node {$\bullet$};
\draw (1,1.4) node {$\bullet$};
\filldraw[ultra thick,color=red] (0.1,0.75) node {$\times$};
\draw (-1,0) node[below right] {$l_n$};
\draw (1,1.4) node[below right] {$u_n$};
\filldraw[color=red] (0.1,0.75) node[above left] {$z_n$};
\end{tikzpicture}
